Ranking Warnings of Static Analysis Tools Using Representation Learning

Static analysis tools are frequently used to detect potential vulnerabilities in software systems. However, an inevitable problem of these tools is their large number of warnings with a high false positive rate, which consumes time and effort for investigating. In this paper, we present DeFP, a novel method for ranking static analysis warnings. Based on the intuition that warnings which have similar contexts tend to have similar labels (true positive or false positive), DeFP is built with two BiLSTM models to capture the patterns associated with the contexts of labeled warnings. After that, for a set of new warnings, DeFP can calculate and rank them according to their likelihoods to be true positives (i.e., actual vulnerabilities). Our experimental results on a dataset of 10 real-world projects show that using DeFP, by investigating only 60% of the warnings, developers can find +90% of actual vulnerabilities. Moreover, DeFP improves the state-of-the-art approach 30% in both Precision and Recall.

==> 3.approach/approach_overview.tex <==
\subsection{Approach Overview}
%
% In this paper, we present \tool, a novel method to rank warnings of static analysis tools. 
% %
% This approach has a great potential because of taking advantage of both program analysis and deep learning technique to exhibit warning's characteristics from raw source code. When compared with other FP detectors, \tool does not require human experts to manually extract hand-engineered features, meaning that FP detection pipeline could be fully automated.

% %
% For each of warnings reported by SA tools, \tool firstly pinpoints the associated statement in the program source code. Rooted from this statement, it slices all the relevant statements that have control or data dependencies for reserving only potential defect code snippets. Afterwards, \tool generalizes the sliced source code by obfuscating all the identifiers (variable names, function names, ...) and embeds it into an initial matrix. Besides, the rooted statement which has warning assigned is independently transformed into numerical space as a second input to train a neural network. By learning from annotated label (TP or FP), a representing model are employed to extract semantic information and infer high-level features from both input matrices. These features are subsequently fed into a machine learning model to better calculate likelihood of the warning to be false positive. Finally, \tool sorts all estimated possibilities and outputs a complete ranked list of warnings.


In this paper, we present \tool, a novel method to rank warnings of SA tools. Our approach takes advantage of both program analysis and deep learning techniques to exhibit warnings' characteristics from source code. Moreover, our approach can be fully automated since it does not require human expert to manually define interesting features. 
Specially, for a set of warnings and the corresponding program source code, \tool outputs a ranked list of warnings which are ordered according to there likelihoods to be TPs. The overview approach of \tool is illustrated in Fig.~\ref{???}.

\begin{enumerate}
    \item \textbf{Learning phase}: From the reported statements, \tool conducts program slicing to extract related statements which are statements impact and be impacted by the reported statements. After that, the reported statements and their slices are tokenized and vectorized into embedding vectors. These vectors are used to trained a XXX model which can capture the meaning of the reported statements, as well as the semantic dependencies of the statements in the slices and then represent them by high-level features. Finally, to better calculate the likelihood to be TPs of warnings,  these features a used to train YYY classifier. The output of this phase is a XXX model and YYY classifier with fine-tune parameters. 
    \item \textbf{Ranking phase}: For a set of warnings and the corresponding program, \tool also conducts program slicing and embeds relevant statements into vectors. After that, the vectors are fed into the model trained in the previous phase. Next, high-level features are extracted by the trained XXX model and scores are predicted by YYY classifier. The output of this phase is a ranked list of warnings.
\end{enumerate}
